Investigating Functional Redundancies in the Context of Vehicle Automation - A Trajectory Tracking Perspective

Level 3+ automated driving implies highest safety demands for the entire vehicle automation functionality. For the part of trajectory tracking, functional redundancies among all available actuators provide an opportunity to reduce safety requirements for single actuators. Yet, the exploitation of functional redundancies must be well argued if employed in a safety concept as physical limits can be reached. In this paper, we want to examine from a trajectory tracking perspective whether such a concept can be used. For this, we present a model predictive fault-tolerant trajectory tracking approach for over-actuated vehicles featuring wheel individual all-wheel drive, brakes, and steering. Applying this approach exemplarily demonstrates for a selected reference trajectory that degradations such as missing or undesired wheel torques as well as reduced steering dynamics can be compensated. Degradations at the physical actuator limits lead to significant deviations from the reference trajectory while small constant steering angles are partially critical.

==> highlight.tex <==
\begin {tabular}{clr<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }r<{\pgfplotstableresetcolortbloverhangright }@{}l<{\pgfplotstableresetcolortbloverhangleft }}%
\toprule \#&Description&\multicolumn {2}{r}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {t,max}}$ \newline in \si {\meter }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {t,avg}}$ \newline in \si {\meter }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {t,end}}$ \newline in \si {\meter }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {n,max}}$ \newline in \si {\meter }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {n,avg}}$ \newline in \si {\meter }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {n,end}}$ \newline in \si {\meter }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {\psi ,max}}$ \newline in \si {\degree }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {\psi ,avg}}$ \newline in \si {\degree }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\varepsilon _{\mathrm {\psi ,end}}$ \newline in \si {\degree }}}&\multicolumn {2}{c}{\parbox {\metricWidth }{\centering $\mathrm {\mu _{avg}}$}}\\\midrule %
(1)&No Degradation&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.34$&\pgfmathparse {int(greater(0.037143,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.037143,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.04$&\pgfmathparse {int(greater(0.000027,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.000027,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(0.051990,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.051990,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.05$&\pgfmathparse {int(greater(0.016469,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.016469,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.02$&\pgfmathparse {int(greater(0.000134,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.000134,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(2.066057,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $2$&\pgfmathparse {int(greater(2.066057,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.07$&\pgfmathparse {int(greater(0.521135,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.521135,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.52$&\pgfmathparse {int(greater(0.000157,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $\textcolor{white}{0}0$&\pgfmathparse {int(greater(0.000157,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&$\textcolor{white}{0}0$&$.40$\\%
(2)&No Degradation, misaligned $m$, $J_z$, \& \cg &\pgfmathparse {int(greater(0.352318,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.352318,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.35$&\pgfmathparse {int(greater(0.055560,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.055560,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.06$&\pgfmathparse {int(greater(0.000070,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000070,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(0.092766,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.092766,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.09$&\pgfmathparse {int(greater(0.030180,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.030180,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.03$&\pgfmathparse {int(greater(0.000080,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000080,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(4.030203,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $4$&\pgfmathparse {int(greater(4.030203,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.03$&\pgfmathparse {int(greater(1.407820,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $1$&\pgfmathparse {int(greater(1.407820,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.41$&\pgfmathparse {int(greater(0.002403,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.002403,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&$0$&$.43$\\%
(3)&$M_{\mathrm {W,rl}}=\SI {500}{\newton \meter }=\mathrm {const.}$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.34$&\pgfmathparse {int(greater(0.038788,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.038788,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.04$&\pgfmathparse {int(greater(0.001053,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.001053,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(0.050524,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.050524,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.05$&\pgfmathparse {int(greater(0.016962,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.016962,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.02$&\pgfmathparse {int(greater(0.000040,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000040,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(2.077887,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $2$&\pgfmathparse {int(greater(2.077887,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.08$&\pgfmathparse {int(greater(0.488560,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.488560,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.49$&\pgfmathparse {int(greater(0.020205,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.020205,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.02$&$0$&$.46$\\%
(4)&$M_{\mathrm {W,rr}}=0=\mathrm {const.}$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.34$&\pgfmathparse {int(greater(0.037188,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.037188,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.04$&\pgfmathparse {int(greater(0.000394,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000394,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(0.051284,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.051284,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.05$&\pgfmathparse {int(greater(0.016305,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.016305,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.02$&\pgfmathparse {int(greater(0.000203,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000203,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(2.063273,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $2$&\pgfmathparse {int(greater(2.063273,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.06$&\pgfmathparse {int(greater(0.501951,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.501951,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.50$&\pgfmathparse {int(greater(0.000632,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000632,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&$0$&$.40$\\%
(5)&$\lambda _{\mathrm {fr}}=\SI {-.13}{}=\mathrm {const.}$&\pgfmathparse {int(greater(0.911243,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.911243,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.91$&\pgfmathparse {int(greater(0.247936,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.247936,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.25$&\pgfmathparse {int(greater(0.062778,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.062778,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.06$&\pgfmathparse {int(greater(0.334236,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.334236,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.33$&\pgfmathparse {int(greater(0.058701,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.058701,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.06$&\pgfmathparse {int(greater(0.000673,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000673,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(15.797356,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $15$&\pgfmathparse {int(greater(15.797356,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.80$&\pgfmathparse {int(greater(3.326127,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $3$&\pgfmathparse {int(greater(3.326127,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.33$&\pgfmathparse {int(greater(0.465707,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.465707,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.47$&$0$&$.76$\\%
(6)&$\lambda _{\mathrm {fr}}=\SI {-1}{}=\mathrm {const.}$&\pgfmathparse {int(greater(5.450440,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $5$&\pgfmathparse {int(greater(5.450440,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.45$&\pgfmathparse {int(greater(0.733564,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.733564,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.73$&\pgfmathparse {int(greater(5.450440,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $5$&\pgfmathparse {int(greater(5.450440,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.45$&\pgfmathparse {int(greater(2.262358,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $2$&\pgfmathparse {int(greater(2.262358,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.26$&\pgfmathparse {int(greater(0.484743,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.484743,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.48$&\pgfmathparse {int(greater(0.750335,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.750335,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.75$&\pgfmathparse {int(greater(27.530889,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $27$&\pgfmathparse {int(greater(27.530889,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.53$&\pgfmathparse {int(greater(6.879764,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $6$&\pgfmathparse {int(greater(6.879764,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.88$&\pgfmathparse {int(greater(14.872692,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $14$&\pgfmathparse {int(greater(14.872692,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.87$&$0$&$.84$\\%
(7)&$\delta _{\mathrm {fr}}\in [\SI {-3}{\degree }, \SI {3}{\degree }]$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.34$&\pgfmathparse {int(greater(0.060307,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.060307,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.06$&\pgfmathparse {int(greater(0.000460,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000460,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(0.234185,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.234185,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.23$&\pgfmathparse {int(greater(0.062354,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.062354,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.06$&\pgfmathparse {int(greater(0.000041,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000041,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(6.415290,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $6$&\pgfmathparse {int(greater(6.415290,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.42$&\pgfmathparse {int(greater(2.309126,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $2$&\pgfmathparse {int(greater(2.309126,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.31$&\pgfmathparse {int(greater(0.065805,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.065805,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.07$&$0$&$.53$\\%
(8)&$\dot {\delta }_{\mathrm {fl}}\in [\SI {-12}{\degree \per \second }, \SI {12}{\degree \per \second }]$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.341718,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.34$&\pgfmathparse {int(greater(0.036326,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.036326,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.04$&\pgfmathparse {int(greater(0.000133,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000133,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(0.073662,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.073662,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.07$&\pgfmathparse {int(greater(0.020049,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.020049,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.02$&\pgfmathparse {int(greater(0.000323,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000323,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(4.036588,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $4$&\pgfmathparse {int(greater(4.036588,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.04$&\pgfmathparse {int(greater(0.988410,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.988410,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.99$&\pgfmathparse {int(greater(0.001887,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.001887,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&$0$&$.40$\\%
(9)&$\delta _{\mathrm {fr}}=0=\mathrm {const.}$&\pgfmathparse {int(greater(0.426756,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.426756,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.43$&\pgfmathparse {int(greater(0.107670,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.107670,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.11$&\pgfmathparse {int(greater(0.004064,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.004064,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(0.740357,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.740357,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.74$&\pgfmathparse {int(greater(0.171349,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.171349,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.17$&\pgfmathparse {int(greater(0.000130,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.000130,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(6.673927,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $6$&\pgfmathparse {int(greater(6.673927,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.67$&\pgfmathparse {int(greater(2.275813,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $2$&\pgfmathparse {int(greater(2.275813,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.28$&\pgfmathparse {int(greater(0.008199,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.008199,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.01$&$0$&$.67$\\%
(10)&$\delta _{\mathrm {fr}}=\SI {-5}{\degree }=\mathrm {const.}$&\pgfmathparse {int(greater(1.068434,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $1$&\pgfmathparse {int(greater(1.068434,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.07$&\pgfmathparse {int(greater(0.499548,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.499548,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.50$&\pgfmathparse {int(greater(0.121201,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.121201,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.12$&\pgfmathparse {int(greater(1.408941,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $1$&\pgfmathparse {int(greater(1.408941,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.41$&\pgfmathparse {int(greater(0.401061,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.401061,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.40$&\pgfmathparse {int(greater(0.001787,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $0$&\pgfmathparse {int(greater(0.001787,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.00$&\pgfmathparse {int(greater(21.584801,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $21$&\pgfmathparse {int(greater(21.584801,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.58$&\pgfmathparse {int(greater(6.231297,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $6$&\pgfmathparse {int(greater(6.231297,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.23$&\pgfmathparse {int(greater(3.569134,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $3$&\pgfmathparse {int(greater(3.569134,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.57$&$0$&$.85$\\%
(11)&$\delta _{\mathrm {fr}}=\SI {-30}{\degree }=\mathrm {const.}$&\pgfmathparse {int(greater(16.775667,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $16$&\pgfmathparse {int(greater(16.775667,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.78$&\pgfmathparse {int(greater(9.009921,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $9$&\pgfmathparse {int(greater(9.009921,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.01$&\pgfmathparse {int(greater(14.809180,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $14$&\pgfmathparse {int(greater(14.809180,1.0))}\ifnum \pgfmathresult =1\boldmath \fi $.81$&\pgfmathparse {int(greater(4.987550,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $4$&\pgfmathparse {int(greater(4.987550,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.99$&\pgfmathparse {int(greater(1.555267,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $1$&\pgfmathparse {int(greater(1.555267,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.56$&\pgfmathparse {int(greater(2.981799,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $2$&\pgfmathparse {int(greater(2.981799,0.3))}\ifnum \pgfmathresult =1\boldmath \fi $.98$&\pgfmathparse {int(greater(43.874774,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $43$&\pgfmathparse {int(greater(43.874774,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.87$&\pgfmathparse {int(greater(13.514476,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $13$&\pgfmathparse {int(greater(13.514476,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.51$&\pgfmathparse {int(greater(17.323271,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $17$&\pgfmathparse {int(greater(17.323271,10.0))}\ifnum \pgfmathresult =1\boldmath \fi $.32$&$0$&$.89$\\\bottomrule %
\end {tabular}%

